Thermal-GEMs: Generalized Models for Building Thermal Dynamics

Data-driven models for building thermal dynamics are a scalable approach for enabling energy-efficient operation through fault detection & diagnosis or advanced control. To obtain accurate models, measurement data from a target building spanning months to years are required. Transfer Learning (TL) mitigates this challenge by employing pretrained models based on single or multiple source buildings. General multi-source TL models promise to outperform single-source TL, but alternative multi-source modeling architectures remain to be explored, and evaluation on real-world data is missing. Moreover, time series foundation models (TSFM) have emerged as candidates for the best-performing general models. Hence, we conduct a first, comprehensive assessment of general modeling approaches for building thermal dynamics, including multi-source TL and TSFMs. Our assessment includes ablations using four state-of-the-art multi-source TL architectures and evaluations on synthetic as well as real-world data. We demonstrate that multi-source TL models are highly effective in accurately modeling buildings in real-world applications, yielding up to 63% lower forecasting errors compared to single-source TL. Moreover, our results suggest a trade-off between multi-source TL models exclusively pretrained with building data and TSFMs pretrained with a multitude of different time series, revealing that data from 16-32 source buildings must be available over 1 year for pretraining multi-source TL models to consistently outperform TSFMs as evaluated using the mean absolute error. These findings provide practical guidance for selecting modeling strategies based on the number of source buildings available for pretraining multi-source TL models.

==> chapters/a1_hyperparam.tex <==
We used Optuna \cite{akiba2019optuna} to tune hyperparameters regarding all general models. Table \ref{tab:z_hyperparam_search_gms} lists all hyperparameter spaces considered in the search for each model. Hyperparameters were tuned for each model on each dataset separately, with 10 trials for each combination. We list all hyperparameters for MSGMs in Table \ref{tab:gm_hyperparams}

\input{tables/z_hyperparam_search_gms}

\input{tables/z_hyperparameter_gm}

==> chapters/a2_additional_results.tex <==
Inthis section, we show additional results, mainly regarding the RMSE metric, which is not vastly thematized in the paper.



\begin{figure*}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figs/01_ss_rmse.pdf}
  \caption{RMSE of Single-Source TL versus MSGM for different fine-tunings on real-world data (Ecobee).}
  \label{fig:appendix_01_ss}
\end{figure*}


\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figs/02_boxplot_rmse.pdf}
  \caption{RMSE performance comparison of the TSFMs against the
best-performing general models.}
  \label{fig:appendix_02_boxplots}
\end{figure}

==> chapters_new/01_introduction.tex <==
Data-Driven Models (DDMs) in buildings are an important pathway towards meeting climate targets. They are widely adopted for applications such as energy-efficient control methods, including Model-Predictive control (MPC) \cite{drgovna2020allyouneedtoknowmpc, balali2023energyddmcontrol, lee2022aimodelwithmpc} and Reinforcement Learning (RL) \cite{arroyo2022rlmpc}. In particular, Machine Learning (ML) models are utilized as DDMs because they exhibit good predictive performance without requiring domain-specific knowledge, as demonstrated for load forecasting \cite{choi2023performance, somu2021electricforecast} and thermal prediction \cite{choi2023performance, elmaz2021cnnlstmforecastthermal} in buildings. However, ML-based models often require months to years of data to achieve satisfying prediction performance \cite{raisch2025cl}. In reality, data availability of less than one year and thus not covering all seasons is common, making accurate models hard to design and train. Additionally, buildings are inherently heterogeneous, meaning each building requires its own specifically fitted DDM. To address these problems, Transfer Learning (TL) approaches have emerged. The main goal of utilizing TL for building thermal dynamics is to use the existing data efficiently to model buildings accurately.
%TL utilizes data from a source building to model a specific target building, thereby addressing the issue of data sparsity.  \\

One data-efficient method to model thermal dynamics in buildings is using Time Series Foundation Models (TSFM). TSFMs are pre-trained on vast amounts of heterogeneous data from different domains to learn efficient representations of temporal patterns. For thermal dynamics in buildings, this was partially explored by \cite{mulayim2024tsfmbuildingsrevolutionize}, as TSFMs can be advantageous in domains with limited available data or different availabilities for features. However, there are two areas underexplored. First, the use of state-of-the-art multivariate TSFM applied to thermal dynamics. But more importantly, TSFMs have not yet been compared to MSGMs for building thermal dynamics, leaving the question open on their effectiveness. \\

\noindent \textbf{Research Question 1:} How do current state-of-the-art TSFMs perform for building thermal dynamics compared to an MSGM approach? \\

In the domain of building thermal dynamics, a single-source TL approach is commonly used \cite{chen2020singlesourcethermal, pinto2022transferleaningsmartbuildingsinglesource}. In single-source TL, a model is pre-trained on a building sharing the same sensors as the source building, and then fine-tuned on the desired target building. Raisch et al. \cite{GenTL2025} were the first to demonstrate a multi-source TL approach. They showed that a multi-source general model (MSGM) outperforms single-source TL for thermal dynamics in buildings. However, a comparison of an MSGM approach to single-source TL based on real-world data for building thermal dynamics is currently unavailable. An evaluation on real-world building data may be crucial to determine the applicability of DDMs, considering that synthetic data for buildings was generated from models that can not replicate the physical system in its entirety \cite{tian2018reviewrealworldbuildings, batty2018digitaltwins}.  \\

\noindent\textbf{Research Question 2:} How does multi-source TL perform compared to a single-source approach for building thermal dynamics on real-world data? \\

In practice, buildings have different types and numbers of sensors and measurement rates. The training of an MSGM, however, requires data from multiple buildings with the same type and amount of sensors with the same measurement rate. For the scope of this paper, we call these buildings \textit{same sensor buildings}.
%This fact requires a dedicated multi-source DDM for each building with a distinct combination of sensors. For the scope of this paper, we call buildings with the same sensor data availability \textit{similar source buildings}. Training MSGMs requires multiple source buildings with the same sensor configuration. 
Because there are many different sensor configurations, it becomes difficult to gather enough same sensor buildings for each sensor combination to train a general model. We refer to this challenge as the \textit{same sensor building sparsity}. This issue is not present for TSFMs, which benefit from large, heterogeneous training corpora across many domains and do not initially require source buildings to achieve reasonable zero-shot performance. Assuming that using more source buildings improves multi-source DDM performance leads to the following unexplored question: \\

\noindent \textbf{Research Question 3:} How many source buildings are needed to train a general model that outperforms current TSFMs? \\

In this paper, we answer the questions by choosing a representative MSGM and TSFMs. For the MSGM, we make an ablation study of four widely used deep learning models. We chose the TSFM by comparing the performance of three different pretrained TSFMs. To ensure that the results are representative, these models are trained and evaluated on three distinct building datasets, which represent more than 500 homes in the US, Canada, the UK, Germany, France, and more. The results should guide the extent to which MSGM should be used for real-world applications in building thermal dynamics. 

% TODO: Change RQ numbers here.
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figs/rq_overview.pdf}
  \caption{Overview of modeling strategies regarding our research questions.}
  \label{fig:rq_overview}
\end{figure}



==> chapters_new/04_experiments.tex <==
This section illustrates the experiments from which we will generate insights to answer our research questions. 
To have an idea of how different architectures for an MSGM perform against the current state-of-the-art TSFMs, we make a large-scale analysis of all models' performances in the experiment \ref{sec:exp1}. Second, we want to answer the question on whether MSGMs help improve the performance of DDMs in comparison to a single-source TL approach for real-world data. For that, we evaluate both on the Ecobee dataset in experiment \ref{sec:exp2} with different ranges of finetuning data available. 
In our last experiment, we then draw a connection between the number of sources used for training a MSGM and its predictive performance. To put the results into context, we use the respective best-performing TSFM for each dataset as a baseline.
All experiments will closely follow the strategies introduced in section \ref{sec:method}. The appendix contains complementary results for each of the experiments.

\subsection{General Models and Foundation Models}
\label{sec:exp1}

In our first experiment, we make an ablation of four general model architectures as MSGMs as described in section \ref{sec:gm_training}. For each model, we performed a hyperparameter tuning with Optuna, which is further detailed in the Appendix. In addition to that, we also evaluated the three TSFMs, Chronos-2, Toto, and TimesFM, and compared their performances against all MSGM architectures.

\begin{figure*}[htbp]
  \centering
 \includegraphics[width=\linewidth]{figs/02_boxplot_mae_all.pdf}
  \caption{Zero-Shot MAE of all MSGMs and TSFMs}
  \label{fig:exp01_gm_zero}
\end{figure*}

The performances of all architectures and TSFMs for all datasets are shown in the box plots of Figure \ref{fig:exp01_gm_zero}. The three leftmost box plots in each bin correspond to the TSFMs, while the rest represent the different MSGM architectures. We observe that overall, the MSGM approach beats the TSFM, with Mamba as an exception to that. In addition to that, the experiment shows that the choice of the TSFM and MSGM architecture only accounts for minor improvements over other options. The performance of the MSGM and TSFM also depends on the Time series they are evaluated on. Counterintuitively, we also observe that the univariate TSFM TimesFM outperforms the multivariate TSFMs on the Ideal set, and Chronos on the Euro set. This can not be expected as the mutivariate TSFMs also have information about external variables, and not only from the indoor temperature, as information available for their predictions.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figs/02_scatter.pdf}
  \caption{Zero-shot performance: Per-building TSFM compared to MSGM (each data point is a target building)}
  \label{fig:exp02_scatter}
\end{figure}

Additionally, we make a direct comparison of Chronos as a representative for the TSFMs with the MSGM approach in Figure \ref{fig:exp02_scatter}. The choice of Chronos was based on the average rank regarding all TSFMs over all datasets; we observed similar results with the other TSFMs. In the figure, each data point represents one building from a dataset, with the color indicating the dataset it stems from, the x coordinate representing the respective error for the MSGM, and the y coordinate for the error of Chronos on it. Points above the red line again indicate that the MSGM made more accurate forecasts on the building than Chronos. The results show that the MSGM is the better choice to model a building than the TSFM regarding both metrics and across all datasets. We observe some exceptions to that for the MAE as the metric, and assume that Chronos potentially performs riskier forecasts, which are potentially not as heavily punished for an MAE compared to the RMSE.

\subsection{Real-World General Models}
\label{sec:exp2}

In the second experiment, we test how well an MSGM approach can model building thermal dynamics in comparison to a single-source approach on the Ecobee dataset as a real-world representative. For the single-source TL, we randomly choose a source from the Ecobee training set and train an LSTM on it. We then iterate over four fine-tuning scenarios: zero-shot, 0.5 months, 1 month, and 2.5  months. For each scenario, we did a seasonal fine-tuning as described in section \ref{sec:seasonal_fineuning} on both the single-source model and the MSGM and reported the average error on the test sets for each of the four seasons, respectively, to ensure robustness in the results.

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figs/01_ss_mae.pdf}
  \caption{MAE of Single-Source TL versus MSGM for different fine-tunings on real-world data (Ecobee). MSGM beats single-source TL once errors are above the dotted line.}
  \label{fig:single-source-gm}
\end{figure*}

Figure \ref{fig:single-source-gm} visualizes the performance of the single-source TL approach in comparison to the MSGM one. Each dot represents one target building from the Ecobee dataset, where the x coordinate represents the MAE of the MSGM and the y coordinate represents the MAE of the single-source TL approach. Both axes are scaled logarithmically for a better representation. A position above the red line indicates that, averaged by season, the MSGM outperformed the single-source approach on the respective building. The results support the intuition that an MSGM approach is not only a valid strategy for simulated buildings but also for real-world scenarios. Across all four data-sparsity scenarios, the MSGM outperformed the single-source TL on every building, with varying improvements. In addition to that, we find that the overall error of the single-source TL decreases with an increasing number of fine-tuning data. Counterintuitively, and contrary to the results of \cite{GenTL2025}, we also observe that on real data, fine-tuning the general model decreases its performance regardless of the number of fine-tuning examples. This may either be an effect of source-buildings that may be less similar to the target buildings or the more rigorous test-error report compared to \cite{GenTL2025}. Consequently, we use the MSGMs in zero-shot mode for further experiments.

\subsection{Transfer Data Sparsity}
\label{sec:exp3}

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=\linewidth]{figs/03_gm_size_mae.pdf}
  \caption{Zero-shot performance: Influence of the number of sources on the MSGM for buildings.}
  \label{fig:03_gm_size}
\end{figure*}

The third experiment dives deeper into the tradeoff between the number of sources used for a general model and its overall performance. One assumption may be that more sources lead to a better performance, which leaves the question open on whether there is a threshold of sources to which a TSFM can outperform a MSGM approach. To test this, we trained multiple MSGMs for each dataset with multiple numbers of sources, ranging from 1 to 128, with power steps of 2. For each number of sources, we first selected this number of sources from the training set of each dataset, respectively, to then train a general model on them. Afterwards, we evaluated this general model on the target set to get an average performance of an MSGM with the respective number of sources.

Figure \ref{fig:03_gm_size} shows the MAE errors of MSGMs with respect to different numbers of sources trained on for all three datasets. For each dataset, we selected the best-performing TSFM regarding the metric used to create a baseline to beat (shown in the top right corner). The results underline the assumption that more sources generally lead to a better performance for the MSGM, with a decreasing return on investment above 64 sources. In addition to that, we observe that for around 16 sources for the Ecobee and Euro dataset and 32 sources for the Ideal dataset, the MSGM consistently begins to perform better than the respective TSFM, beating the benchmark on average. Deviations from that can be seen, for instance, at 32 sources for the Ecobee dataset, which we attribute to an unfavourable random selection of sources. For the Ideal dataset, it has to be added that for the random selection of sources, it could occur that different rooms of the same building could have been selected, leading to more homogeneous sources. This effect may lead to an increased number of sources needed to beat the TSFM baseline.

==> tables/european_houses_distribution.tex <==
\begin{table}[h!]
\centering
\caption{Variation Parameter for buildings in the European Households dataset.}
\label{tab:european_variations}
\begin{tabular}{l|c|c}
\toprule
\textbf{Parameter} & \textbf{Values} & \textbf{\# Variations} \\
\midrule
$U_\text{wall}$ [W/(m$^2$K)]   & $\{0.1, 0.4, 0.7, 1, 1.3\}$  & 5   \\
$c_\text{wall}$ [kJ/(m$^2$K)]  & $\{30, 165, 300\}$           & 3   \\
$f_\text{win}$ [-]             & $\{0.15, 0.2\}$              & 2   \\
$A_\text{ground}$ [m$^2$]      & $\{60, 90, 120\}$            & 3   \\
\midrule
\multicolumn{2}{c|}{\textbf{Total Building Variations}} & \textbf{90} \\
\bottomrule
\end{tabular}
\end{table}

==> tables/fms.tex <==
\begin{table}[h!]
\centering
\caption{List of all foundation models used}
\label{tab:fms}
\begin{tabular}{l | c | c | c}
\toprule
\textbf{Model} & Chronos-2 \cite{ansari2025chronos2} & Toto \cite{cohen2025toto} & TimesFM \cite{das2024timesfm} \\
\hline
%\textbf{Train Data} & Real + Synth & Real + Synth & Real + Synth \\
\# \textbf{Params} & 120M & 151M & 200M \\
\textbf{Architecture} & Encoder & Decoder & Decoder  \\
\textbf{Forecast} & Multivariate & Multivariate & Univariate \\
\bottomrule
\end{tabular}
\end{table}

==> tables/gm_hyperparams.tex <==
\begin{table}[h!]
\centering
\caption{Hyperparameter for the General Models.}
\label{tab:gm_hyperparams}
\begin{tabular}{l | c | c | c | c | c}
\toprule
\textbf{Hyperparameter} & \textbf{A1} & \textbf{A2} & \textbf{A3} & \textbf{A4} & \textbf{A5} \\
\hline \hline
Hidden Size & 192 & 192 & 192 & 128 & 192 \\
\# Layers & 3 & 4 & 4 & 4 & 5 \\
\hline
Optimizer & Adam & Adam & Adam & Adam & Adam \\
Use AMP & True & True & True & True & False \\
Batch Size & 64 & 64 & 64 & 64 & 64 \\
Learning Rate & 0.001 & 0.0005 & 0.0001 & 0.0001 & 0.0005 \\
Dropout & 0.0 & 0.0 & 0.0 & 0.0 & 0.0  \\
\hline
\# Attention Heads & - & 4 & 4 & - & - \\
\bottomrule

\end{tabular}
\end{table}
